(Learned) Frequency Estimation Algorithms under Zipfian Distribution

\begin{abstract} The frequencies of the elements in a data stream are an important statistical measure and the task of estimating them arises in many applications within data analysis and machine learning. Two of the most popular algorithms for this problem, Count-Min and Count-Sketch, are widely used in practice. In a recent work [Hsu et al., ICLR'19], it was shown empirically that augmenting Count-Min and Count-Sketch with a machine learning algorithm leads to a significant reduction of the estimation error. The experiments were complemented with an analysis of the expected error incurred by Count-Min (both the standard and the augmented version) when the input frequencies follow a Zipfian distribution. Although the authors established that the learned version of Count-Min has lower estimation error than its standard counterpart, their analysis of the standard Count-Min algorithm was not tight. Moreover, they provided no similar analysis for Count-Sketch. In this paper we resolve these problems. First, we provide a simple tight analysis of the expected error incurred by Count-Min. Second, we provide the first error bounds for both the standard and the augmented version of Count-Sketch. These bounds are nearly tight and again demonstrate an improved performance of the learned version of Count-Sketch. In addition to demonstrating tight gaps between the aforementioned algorithms, we believe that our bounds for the standard versions of Count-Min and Count-Sketch are of independent interest. In particular, it is a typical practice to set the number of hash functions in those algorithms to $\Theta (\log n)$. In contrast, our results show that to minimize the \emph{expected} error, the number of hash functions should be a constant, strictly greater than $1$.

==> abstract.tex <==
\begin{abstract}
The frequencies of the elements in a data stream are an important statistical measure and the task of estimating them arises in many applications within data analysis and machine learning. 
Two of the most popular algorithms for this problem are Count-Min and Count-Sketch that hash the elements from the stream to a set of buckets. Using a function of the frequencies of items colliding with a query item they estimate the frequency of the query item.  
%A classic algorithm for the problem, Count-Min, hashes the elements from the stream to a set of buckets, keeps track of the total number of items hashing to each bucket, and uses these values as frequency estimates. 

In a recent work [Hsu et al., ICLR'19], it was shown empirically that by augmenting Count-Min and Count-Sketch with a machine learning algorithm for detecting heavy hitters and store these in separate buckets, the approximation error was reduced. The experiments were complemented with an analysis of the expected error incurred by Count-Min when the input has a Zipfian distribution, both in its standard implementation and when augmented by a perfect oracle for detecting heavy hitters. Although the authors established an improved performance of the learned version of Count-Min, their analysis of the standard Count-Min for Zipfians is not tight. Moreover, they provide no similar analysis for Count-Sketch.

In this paper we resolve this problem by first providing a simple tight analysis of the expected error incurred by Count-Min when the input has a Zipfian distribution. Second, we provide the first error bounds for both a standard and learning augmented implementation of Count-Sketch when the input has a Zipfian distribution. These bounds are nearly tight and again demonstrate an improved performance of the learned version of Count-Sketch. 

We believe that our bounds for the standard versions of Count-Min and Count-Sketch are of independent interest. For a high probability error bound on the estimates, the number of hash functions is normally selected as $\Theta (\log n)$. Our results show that to minimise the \emph{expected} error the number of hash functions should be a constant (strictly greater than $1$). 
%Our methods exploit the techniques from ...  
%\todo{Feel free to change this. I just wanted to get started}

%The idea of augmenting classical algorithm with machine learning oracles/advice in a way that existing worst-case guarantees are preserved could be of independent interest.
\end{abstract}

==> lookup.tex <==
\section{Lookup model}\label{sec:lookup}
Another way of obtaining information about heavy hitters in a stream is to create a lookup table of potential heavy hitters based on the heavy hitters in a prefix of the string. For a prefix to be representative we will need some independence between the elements in the stream. To be precise we assume that the stream has the form $(a_1,\dots,a_m)$ where the $(a_j)_{j\in [m]}$ are independent random variables with $\Pr[a_j=i]= \frac{f_i}{\sum_{k=1}^nf_k}$ for each $j\in [m]$ and $i\in [n]$. Our algorithm proceeds by finding the heavy hitters in a ``prefix'' $(s_1,\dots,s_{S})$ of length $S$, where the $s_j$'s are mutually independent of the $a_j$'s and of each other and have the same distribution as the $a_j$'s. Let $A_i=\{j\in S:a_j=i\}$ for $i \in [n]$. For some threshold $T\in \N$, $i$ is characterized as a heavy hitter if $|A_i|\leq |A_j|$ for at most $T$ choices of $j\in [n]$, that is, if $i$ is among the $T$ most frequent items in $S$, and we denote this event $\mathcal{D}_i$

\begin{lemma}\label{lemma:notdetected}
For $i\leq T/2$, it holds that
\begin{align}\label{eq:detecti}
\Pr[\overline{\mathcal{D}_i}]= \exp\left(-\Omega \left(\frac{S}{iH_n}\right)\right).
\end{align}
\end{lemma}
\begin{proof}
Let $i\leq T/2$ be fixed and note that $\E[|A_i|]=\frac{S}{iH_n}$. For $j\in [n]$ let $\mathcal{E}_j$ denote the event that $|A_j|\geq |A_i|$. We will now upper bound the probability of $\mathcal{E}_j$ for fixed $j>\frac{3}{4}T$. 
Define the event $\mathcal{A}=(|A_i|\leq \frac{3}{4}\E[|A_i|)$.
By a standard Chernoff bound
\begin{align}\label{eq:ibad}
\Pr \left[\mathcal{A} \right]=\exp \left(-\Omega \left( \frac{S}{i H_n} \right)\right).
\end{align}
Define the random variable $X_{\ell}^{(j)}=[a_\ell=j]$ for $\ell\in [S]$ and $X^{(j)}=\sum_{\ell\in [S]}X_\ell^{(j)}$. Note that $\frac{3}{4i}-\frac{1}{j}>\frac{3}{4i}-\frac{4}{3T}\geq \frac{3}{4i}-\frac{2}{3i}\geq \frac{1}{12i}>0$ by our assumptions on $i$ and $j$. Furthermore $\Var[X^{(j)}]\leq \E[X^{(j)}]= \frac{S}{jH_n}$ so by Bennett's inequality


\begin{align}
&\Pr\left[X^{(j)} \geq\frac{3}{4}\E[A_i]\right]= \Pr\left[X^{(j)} -\E[X^{(j)}]>\frac{S}{H_n}\left(\frac{3}{4i}-\frac{1}{j}\right)\right]\leq \exp\left(-\frac{S}{jH_n} h \left(\frac{j}{12i} \right)\right) \nonumber \\
\leq &\exp\left(-\frac{S}{24iH_n} \log \left(1+\frac{j}{12i} \right) \right) 
=\exp\left(-\Omega\left(\frac{S}{iH_n} \log \left(\frac{j}{i} \right) \right) \right)=\left( \frac{i}{j} \right)^{\Omega \left(\frac{S}{iH_n} \right)}. \label{eq:jdomi}
\end{align}
Now for $\frac{3}{4}T <j \leq n$ define the random variable $Z_j=\left[X^{(j)} \geq\frac{3}{4}\E[A_i]\right]$ and $Z=\sum_{\frac{3}{4}T <j \leq n}Z_j$. If $\overline{\mathcal{D}_i}$ occurs then either $\mathcal{A}$ occurs or $|A_j| \geq\frac{3}{4}\E[A_i]$ for at least $T$ values of $j$ and in particular $Z\geq \frac{T}{4}$. Thus by a union bound
\begin{align}\label{eq:unionbound}
\Pr[\overline{\mathcal{D}_i}]\leq \Pr[\mathcal{A}]+\Pr\left[Z \geq \frac{T}{4}\right].
\end{align}
We proceed to upper bound $\Pr\left[Z \geq \frac{T}{4}\right]$. Let $c>0$ be the implicit constant in~\eqref{eq:jdomi} and assume with no loss of generality that $S$ is such that $c\frac{S}{iH_n}\geq 5$ (if not,~\eqref{eq:detecti} holds trivially). Then
$$
\E[Z]\leq \sum_{\frac{3}{4}T<j\leq n} \left( \frac{i}{j} \right)^{c\frac{S}{iH_n}}
\leq \frac{3T}{4} \left(\frac{4i}{3T} \right)^{c\frac{S}{iH_n}}
\leq \frac{3T}{4} \left( \frac{2}{3}\right)^{c\frac{S}{iH_n}}<\frac{T}{8}.
$$ 
As let $\sigma^2=\Var[Z]\leq \E[Z]$. It follows by Bennett's inequality that 
\begin{align*}
\Pr\left[Z \geq \frac{T}{4}\right]&\leq \Pr\left[Z-\E[Z] \geq \frac{T}{8}\right]
\leq \exp \left(-\sigma^2 h \left( \frac{T}{8 \sigma^2} \right) \right)
\leq \exp \left(-\frac{T}{16} \log \left(1+\frac{T}{8 \sigma^2} \right) \right) \\
& \leq \exp \left(-\frac{T}{16} \log \left(1+\frac{1}{6}\left(\frac{3T}{4i} \right)^{c\frac{S}{iH_n}} \right) \right)
= \exp \left(- \Omega \left(\frac{TS}{iH_n}\right) \right) 
\end{align*}
Combining this with~\eqref{eq:ibad} and~\eqref{eq:unionbound} gives the desired result.
\end{proof}
\subsection{Lookup Count-Min}
\Cref{lemma:notdetected} provides an upper bound on the probability that item $i$ is not detected as a heavy hitter. The following theorem follows easily.
\begin{theorem}
Let $T\leq B/2\leq n/6$ and suppose we implement Count-Min with a lookup table of size $T$ for storing the heavy hitters characterized from a prefix of length $S=C\cdot T \log n$ for some sufficiently large constant $C$. Let  $Z=\sum_{i\in [n]}f_i|\tilde{f_i}-f_i|$. Then 
$$
\E[Z]=O\left(\frac{\log \left(\frac{n}{B} \right)\log \max\left\{\frac{n}{T},\frac{nH_n}{S} \right\}}{B}  \right).
$$
\end{theorem}
The maximum in the bound from the theorem may seem confusing but a little thought reveals that it is natural: If $S\geq TH_n$ then we expect to detect at least $S/H_n\geq T$ heavy hitters but we have only $T$ cells to store them and this gives rise to the $\log(n/T)$ term. If on the other hand $S< TH_n$ we have plenty of cells to store the heavy hitters but we only detect $S/H_n$ which gives rise to the $\log (nH_n/S)$ term. In practice we would of course set $S$ and $T$ such that $S=\Theta(H_n T)$ and then the expression for $\E[Z]$ above becomes simpler.
\begin{proof}
Suppose that item $i$ is not characterized as a heavy hitter. Imitating the proof of~\Cref{thm:simplecm} we obtain that $\E[|\tilde{f_i}-f_i|]=O \left( \frac{\log(n/B)}{B}\right)$. Letting $\mathcal{D}_i$ denote the event that item $i$ is characterized as a heavy hitter it thus holds that
$$
\E[Z]= O\left(\frac{\log(n/B)}{B}\sum_{i=1}^n f_i\Pr[\overline{\mathcal{D}_i}] \right).
$$
Let $c>0$ be the implicit constant in~\Cref{lemma:notdetected}. Assuming first that $S\geq T H_n$ we obtain using the lemma that
$$
\sum_{i=1}^n f_i\Pr[\overline{\mathcal{D}_i}]\leq \sum_{i\leq T/2}f_i\exp\left(-c\frac{S}{iH_n}\right)+\sum_{T/2<i\leq n}f_i=O\left(\log (n/T)\right).
$$
If on the other hand $S<TH_n$ we obtain that 
$$
\sum_{i=1}^n f_i\Pr[\overline{\mathcal{D}_i}]\leq \sum_{i\leq S/H_n}f_i\exp\left(-c\frac{S}{iH_n}\right)+\sum_{S/H_n<i\leq n}f_i=O\left(\log \left(\frac{nH_n}{S}\right)\right).
$$
The result follows.
\end{proof}
\subsection{Lookup Count-Sketch}
